Temporal Grounding Graphs for Language Understanding with Accrued Visual-Linguistic Context

A robot's ability to understand or ground natural language instructions is fundamentally tied to its knowledge about the surrounding world. We present an approach to grounding natural language utterances in the context of factual information gathered through natural-language interactions and past visual observations. A probabilistic model estimates, from a natural language utterance, the objects,relations, and actions that the utterance refers to, the objectives for future robotic actions it implies, and generates a plan to execute those actions while updating a state representation to include newly acquired knowledge from the visual-linguistic context. Grounding a command necessitates a representation for past observations and interactions; however, maintaining the full context consisting of all possible observed objects, attributes, spatial relations, actions, etc., over time is intractable. Instead, our model, Temporal Grounding Graphs, maintains a learned state representation for a belief over factual groundings, those derived from natural-language interactions, and lazily infers new groundings from visual observations using the context implied by the utterance. This work significantly expands the range of language that a robot can understand by incorporating factual knowledge and observations of its workspace in its inference about the meaning and grounding of natural-language utterances.

==> figure-generation-files/figure-generation.tex <==
%%%%% Figure related.
\newcommand{\subdiag}[7]{%
  \node[#7, #1=of #2t, xshift=#3cm, yshift=#4cm] (#5t) {$#6{t}$};
}
\newcommand{\subdiagX}[7]{%
  \node[#7, #1=of #2t, xshift=#3cm, yshift=#4cm] (#5t) {$#6{0:t}$};
}
 
\renewcommand{\subdiag}[7]{%
   \node[#7, #1=of #2t1, xshift=#3cm, yshift=#4cm] (#5t1) {$#6{1}$};
   \node[#7, #1=of #2tn1, xshift=#3cm, yshift=#4cm] (#5tn1) {$#6{t-1}$};
   \node[#7, #1=of #2t, xshift=#3cm, yshift=#4cm] (#5t) {$#6{t}$};
 }
 \tikzset{
     between/.style args={#1 and #2}{
          at = ($(#1)!0.5!(#2)$)
     }
   }
 
 \begin{tikzpicture}
   %
   \node[obs] (kb0) {$\KB{0}$};
   \node[latent, right=of kb0, xshift=1.6cm] (kb1) {$\KB{1}$};
   \node[latent, right=of kb1, xshift=1.6cm] (kbtn2) {$\KB{t-2}$};
   \node[latent, right=of kbtn2, xshift=1.6cm] (kbtn1) {$\KB{t-1}$};
   \node[latent, right=of kbtn1, xshift=1.6cm] (kbt) {$\KB{t}$};
   % %
   \factor[between=kb0 and kb1, xshift=0.1cm] {ft1} {} {} {};
   \factor[between=kbtn2 and kbtn1, xshift=0.1cm] {ftn1} {} {} {};
   \factor[between=kbtn1 and kbt, xshift=0.1cm] {ft} {} {} {};
   \draw[dashed] (kb1) -- (kbtn2);
   % %
   \subdiag{below}{f}{0}{0}{c}{\Correspondences}{latent}
   % %
   \factoredge {kb0, kb1, ct1} {ft1} {};
   \factoredge {kbtn2, kbtn1, ctn1} {ftn1} {};
   \factoredge {kbtn1, kbt, ct} {ft} {};
   % %
   \subdiag{below}{f}{-0.8}{0.6}{gr}{\Grounding}{obs}
   \subdiag{below}{c}{1.2}{0.6}{ac}{\Action}{latent}
   \subdiag{below}{c}{-0.2}{0.3}{la}{\Language}{obs}
   \subdiag{below}{c}{-2.0}{-0.8}{vo}{\VisualObservations}{obs}
   % %
   \factor[below=0.8 of grt1, xshift=0.0cm] {mt1} {} {} {};
   \factor[below=0.8 of grt, xshift=0.0cm] {mt} {} {} {};
   \factor[below=0.8 of grtn1, xshift=0.0cm] {mtn1} {} {} {};
   % %
   \factoredge {grt1,lat1,vot1,ct1,kb0} {mt1} {};
   \factoredge {grt,lat,vot,ct,kbtn1} {mt} {};
  \factoredge {grtn1,latn1,votn1,ctn1,kbtn2} {mtn1} {};
  % %
  \factor[right=0.1 of ct1, yshift=-0.5cm] {pl1} {} {} {};
  \factor[right=0.1 of ct, yshift=-0.5cm] {pl} {} {} {};
  \factor[right=0.1 of ctn1, yshift=-0.5cm] {pln1} {} {} {};
  % %
  \factoredge {ct1,act1} {pl1} {};
  \factoredge {ct,act} {pl} {};
  \factoredge {ctn1,actn1} {pln1} {};
  % %
  \node (gt1) [rounded corners, dashed, draw=red, fit= (vot1) (votn1), inner sep=0.12cm] {};
  \node (gt) [rounded corners, dashed, draw=red, fit= (vot1) (vot) (votn1), inner sep=0.18cm] {};
\end{tikzpicture}


==> sections/background.tex <==
% Problem formulation.
\section{Background}
\label{sec:background}

%% Introduce preliminaries.
% Control 
Consider a robot manipulator capable of executing a control sequence 
$\Control$ comprising of future actions $\{ \ControlInitial, \dots, \ControlFinal \}$ 
initiated at time $t$. 
% Workspace.
The operating workspace consists of rigid bodies that may be 
manipulated by the robot or other agents such as the human operator. 
% Visual sensor.
The robot observes its workspace through a visual sensor that captures 
imagery and metric depth information for localization within its environment.
% World model.
The robot's world model, $\WorldModel{t}$  
consists of the set of objects $(o \in \mathcal{O})$ with associated pose information, 
typically obtained from a perception system. 
% Language
The human operator communicates with the robot through a natural language interface 
(via speech or text input). 
Let $\Language{t}$ denote the input language utterance at time $t$ 
composed of a set of constituents $\{\Phrase{1}^{t}, \dots, \Phrase{n}^{t}\}$.
% Estimating trajectory. 
Estimating the control sequence that satisfies the command 
in the context of the current world state can be posed as:
% Estimating actions directly.
\begin{equation} \label{eq:gnd-motion}
\begin{split}
\Control^{*} = 
%\underset{ \Control \in \mathcal{R}^{\mathcal{C}} }{\arg\max} \hspace{1mm}
\underset{ \Control }{\arg\max} \hspace{1mm}
 P( \Control | \Language{t}, \WorldModel{t} ).
\end{split}
\end{equation}

% Groundings.
It is assumed that the language command expresses semantic concepts derived 
from the world model or high-level actions that the robot must perform. 
% Predicates
Contemporary approaches use a set of predicate symbols to express 
semantic concepts that embody attributes and relations that are true 
in the environment. These include notions such as object, spatial relations, 
as well as  high-level actions such as picking or placing that the robot can perform.
% Space of symbols
The full space of predicates that may be true of an environment forms the 
space of groundings $\Grounding{t}(\WorldModel{t})$. 
%
Following \cite{tellex2011understanding, howard2014efficient, Paul-RSS-16}, 
the task of understanding language commands is posed as 
relating each linguistic component in the command with a likely grounding. 
This is posed as estimating binary correspondence variables 
$(\CV{i} \in \Correspondences{t})$ that express the degree to which 
a linguistic constituent $(\Phrase{i} \in \Language{t})$ maps to a concept $(\GV{i} \in \Grounding{t})$.
The estimated set of true correspondences yields the likely meaning or ``groundings''
for an input instruction. 
%Estimating correspondences distill the meaning embedded in the language input and 
The problem of following instructions can hence be formulated as: 
% Introduce Gnd. 
\begin{equation} \label{eq:gnd-motion}
\begin{split}
 P( \Control, \Correspondences{t} ) = 
 \Integral{ \Correspondences{t}}
 P( \Control | \Correspondences{t} ) 
 P( \Correspondences{t} | \Language{t}, \Grounding{t}(\WorldModel{t}) ).
\end{split}
\end{equation}
% What CVs do.
The knowledge of correspondence variables decouples the 
action generation and command understanding inference. Given the 
grounding for the command, the optimal control sequence ($\Control^{*}$) can be generated 
via a platform-specific planning algorithm. 
% Remainder.
In the remainder of this paper, we refer to estimated correspondences 
to imply the set of true groundings for the input instruction, where 
the space of possible groundings is determined as a function of the world model.  
% Limitations of contemporary models.
Contemporary models interpret instructions based on a world 
representation derived from current observations. Hence, are unable to ground 
instructions that refer to semantic information embedded in past observations 
or language inputs. We formalize the problem in the next section and 
present the probabilistic model subsequently.





==> sections/complexity-analysis-backup.tex <==
\subsection{Complexity Analysis}

\begin{table*}[t!]
  \begin{center}
    \caption[h]{$O$-bounds on the asymptotic complexity of different approaches to state keeping with Temporal Grounding Graphs.}
    \begin{tabular}{lccc}
      & No state keeping & Proposed approached & Full state keeping \\
      Observations at each inference step & $\{ \Language{0:t}, \VisualObservations{0:t} \}$ & $\VisualObservations{0:t}$ & $\varnothing$  \\
      State maintained after each inference & $\varnothing$ & $\Gamma^{\mathcal{F}}$ & $\Gamma^{\mathcal{P}}\cup\Gamma^{\mathcal{F}}$ \\
      Space complexity & $\mathbb{\Lambda}t+\mathbb{Z}t$ & $\mathbb{\Gamma}^{\mathcal{F}}\mathbb{o}t$ & $\mathbb{\Gamma}^{\mathcal{P}}\mathbb{o}^{C_{\Lambda}C_{w}}t+\mathbb{\Gamma}^{\mathcal{F}}\mathbb{o}t$\\
      Grounding time & $t{C_{w}}^{t\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda}$ & $t{C_w}^{\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda}$ & ${C_w}^{\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda}$\\
    \end{tabular}
    \label{tab:complexity}
  \end{center}
\end{table*}

The approach presented here relies on minimalistic state keeping in the sense
that we keep a partial state which trades off the runtime of grounding a single
command with the space and time complexity of analyzing visual observations.
%
This is summarized by Table \ref{tab:complexity} in which we provide a
comparison of our approach with two common alternatives, relying entirely on
observations without any state keeping and keeping a full symbolic state; where
$\mathbb{\Lambda}$ and $\mathbb{Z}$ are the worst case longest sentence and
video requiring the most number of detections, $C_W$ is the word with the
largest state space, $C_\Lambda$ is the number of participants the in event
described by the the worst case sentence, $\mathbb{\Gamma}^{\mathcal{F}}$ and
$\mathbb{\Gamma}^{\mathcal{P}}$ are the number of the factual and perceptual
grounding predicates, and $\mathbb{o}$ is the number of possible object
instances.
%
Not keeping any state results in low space complexity
$O(\mathbb{\Lambda}t+\mathbb{Z}t)$, while having high grounding time complexity
$O(t{C_{w}}^{t\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda})$, note the exponential
dependency on $t$, the number of time steps.
%
Reasoning about any new sentence requires re-reasoning about all previously seen
sentences and any correlations between those sentences resulting in an
exponentially increasing joint distribution.
%
Even for short exchanges this runtime is infeasible.

Conversely, keeping all perceptual state in a symbolic manner results in
extremely efficient inference of groundings,
$O({C_w}^{\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda})$.
%
The likelihoods of any declarative groundings are already recorded and only
groundings which are relevant to the given command must be updated from time
$t-1$ to $t$.
%
Yet this process must record all possible inferences for any grounding in any
previous observation so they can be available for grounding when the stimulus is
discarded.
%
Doing so is prohibitively expensive,
$O(\mathbb{\Gamma}^{\mathcal{P}}\mathbb{o}^{C_{\Lambda}C_{w}}t+\mathbb{\Gamma}^{\mathcal{F}}\mathbb{o}t)$,
due to the arity of groundings; even a binary grounding requires storing a fact
about every pair of possible objects.

We strike a middle ground between these alternatives by taking advantage of two
facts.
%
First, any one sentence requires a small number of declarative groundings which
can be estimated using prior visual observations in time linear in the size of
those observations.
%
Second, storing factual groundings removes the need to rerun inference over
prior utterances dramatically speeding up grounding time to
$O(t{C_w}^{\mathbb{\Lambda}}\mathbb{Z}^{C_\Lambda})$, note the lack of $t$ as an
exponent while adding only a small amount of storage,
$O(\mathbb{\Gamma}^{\mathcal{F}}\mathbb{o}t)$ increasing by a constant factor
with each new sentence,
%
This is what we mean by a minimalistic store, we revert to using the stimulus to
save on exponential blowup in storage needs and record facts to lower the
exponent of inferring groundings.

\if 0
Approach that maintains all observations, no state $P(\Phi_{t} | \Lambda_{0:t}, Z_{0:t} )$. This leads to high inference cost trading low space complexity. 
Maintaining and propagating all groundings leads to the following factorization:  $P(\Phi_{t} | \Lambda_{t}, Z_{t}, \nu_{t-1} ) P(\nu_{t-1} | \Lambda_{0:t-1}, Z_{0:t-1})$. 
Our approach attempts to balance the two ends of the spectrum. We estimate the following: $P(\Phi_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} ) P(\nu_{t-1} | \Lambda_{0:t-1}, Z_{0:t-1})$. 
Key idea: the space of factual groundings is smaller compared to perceptual groundings. Hence maintain factual groundings and infer perceptual groundings backwards. 
Inference is exponential in the size of the sentence (each grounding can potentially be correlated to all others), hence reducing the number of phrases reduce complexity 
by a constant factor. Note, we cannot maintain all since space of perceptual groundings is large.
Note: need to update the ST equations and explain the notation below.
\fi

\if 0
% Tables for complexity analysis
\begin{table*}[t]
\begin{center}
\caption[h]{Complexity Analysis for State Representations }
  \begin{tabular}{ | l | l | l | l |}
    \hline
    							& 	All Observations								&	Full State																&	Proposed \\ \hline
    Observations 				&	\text{Full} $\{ \Language{0:t}, \VisualObservations{0:t} \}$	& 	\text{None} $\{ \varnothing \}$												&	\text{Visual} $\{ \VisualObservations{0:t} \}$ \\ %\hline
    Propagated State				& 	\text{None} $\{ \varnothing \}$						&	\text{Full} $ \{ \Gamma^{\mathcal{P}} \cup \Gamma^{\mathcal{F}} \}$					&	\text{Factual} $ \{ \Gamma^{\mathcal{F}} \}$ \\ \hline
    Context (Space Complexity) 		& 	\text{Const.} $O\big( ( | \Lambda | + | Z | ) . t \big)$ 		&	\text{Exp.} $O \big( ( | \Gamma^{\mathcal{P}} | . 2^{| \mathcal{O} |} + \Gamma^{\mathcal{F}}).t \big)$ 	& \text{Linear} $O(\Gamma^{\mathcal{F}}.t)$ \\ %\hline
    Inference (Time Complexity) 	 	& 	\text{Exp.} $ O( c^{t. (\Gamma^{P} + \Gamma^{F} + \Gamma^{\pi}) }.| Z |^{|\mathcal{O}|} ) $		& 	\text{Const.} $ O( c^{ \hat{\Gamma^{\pi}} } )$		&	\text{Exp. reduced} $O(c^{ \hat{\Gamma^{\pi}} + \hat{\Gamma^{P}} }. | Z |^{|\mathcal{O}|} ) $ \\ \hline
  \end{tabular}
\end{center}
\end{table*}


\begin{comment}
% Tables for complexity analysis
\begin{table*}
\begin{center}
\caption[h]{Complexity Analysis for State Representations }
  \begin{tabular}{ | l | l | l | l |}
    \hline
    Approach					& 	All Observations							&	Full State																&	Proposed \\ \hline
    Observations 				&	$\{ \Language{0:t}, \VisualObservations{0:t} \}$		& 	$\{ \varnothing \}$														&	$\{ \VisualObservations{0:t} \}$ \\
    State						& 	\text{None} $\{ \varnothing \}$					&	$ \Gamma^{\mathcal{P}} \cup \Gamma^{\mathcal{F}}$							&	$\Gamma^{\mathcal{F}}$ \\
    Context (Space Complexity) 		& 	$O\big( ( | \Lambda | + | Z | ) . t \big)$ 			&	$O \big( ( | \Gamma^{\mathcal{P}} | . 2^{| \mathcal{O} |} + \Gamma^{\mathcal{F}}).t \big)$ 	& 	$O(\Gamma^{\mathcal{F}}.t)$ \\
    Inference (Time Complexity) 	 	& 	$ O( c^{t. (\Gamma^{P} + \Gamma^{F} + \Gamma^{\pi}) }.| Z |^{|\mathcal{O}|} ) $		& 	$ O( c^{ \hat{\Gamma^{\pi}} } )$		&	$O(c^{ \hat{\Gamma^{\pi}} + \hat{\Gamma^{P}} }. | Z |^{|\mathcal{O}|} ) $ \\
    \hline
  \end{tabular}
\end{center}
\end{table*}
\end{comment}
\fi

==> sections/factors-dcg.tex <==
% DCG Factor
\subsection{ Distributed Correspondence Graphs }
Factor. $ \Psi( \Imp{ \Correspondences{t} }, \Imp{ \Language{t} }, \Dec{ \Correspondences{t} }, \WorldModel{t} ) $

% Declarative factor: factorisation over the phrases.
\begin{equation} \label{eq:imp-language-factorisation}
\begin{split}
P( \Imp{ \Correspondences{t} } |  \Imp{ \Language{t} }, \Dec{ \Correspondences{t} }, \WorldModel{t} ) = 
  \prod_{i = 1}^{ \Imp{n} }
    P( \Imp{ \CV{i} } | \Imp{ \Phrase{i} }, \Imp{ \GV{i} }, \Imp{ \Grounding{c_{i} } }, \Dec{ \Correspondences{} }, \WorldModel{t} )
\end{split}
\end{equation}

% Factored over groundings.
\begin{equation} \label{eq:imp-cv-full}
\begin{split}
P( \Imp{ \Correspondences{t} } |  \Imp{ \Language{t} }, \Dec{ \Correspondences{t} }, \WorldModel{t} ) = 
  \prod_{i = 1}^{ \Imp{n} }
  \prod_{j = 1}^{ \Imp{ \Grounding{} } (\WorldModel{t}) }
    P( \Imp{ \CV{ij} } | \Imp{ \Phrase{i} }, \Imp{ \GV{ij} }, \Imp{ \Grounding{c_{ij} } }, \Dec{ \Correspondences{} }, \WorldModel{t} )
\end{split}
\end{equation}

Show a factor graph. Talk about constraints. Add a statement on the plannner. 



==> sections/factors-grounding-model.tex <==
% Grounding model.
\subsubsection{Declarative Grounding Model}
% Sentence Tracker
%\subsubsection{Declarative Grounding Model}
The declarative grounding model, $P( \Dec{ \Correspondences{t} } | \Dec{ \Language{t} }, \VisualObservations{0:t}, \KB{t\text{-}1})$, 
can be expressed as two conditionals estimating perceptual and declarative groundings as follows:
% Declarative factor: factorisation-three-terms
\begin{equation} \label{eq:factorization-three-terms}
\begin{split}
P( \Dec{ \Correspondences{t} } |  \Dec{ \Language{t} } , \VisualObservations{0:t}, \KB{t-1} ) = 
    \overbrace{
    P( \Correspondences{t}^{\mathcal{F}} | \Dec{\Language{t}}, \KB{t-1})
     }^{\text{Factual Grounding}}
    \overbrace{
    P( \Correspondences{t}^{\mathcal{P}} | \Dec{ \Language{t}}, \VisualObservations{0:t} )
     }^{\text{Perceptual Grounding}}
%    \overbrace{
%    P( \WorldModel{t} | \Dec{ \Language{t}}, \VisualObservations{0:t} )
  %  }^{\text{Object Tracking}}
\end{split}
\end{equation}
%
The grounding likelihoods $P( \Correspondences{t}^{\mathcal{F}} | \Dec{\Language{t}}, \KB{t-1})$
 for factual concepts are derived from the state variable $\KB{t-1}$ containing the marginal distribution over 
 facts from past language inputs. 
 
The inference over spatial relations, entity attributes and events or actions relies on the time 
ordered set of observations $P( \Correspondences{t}^{\mathcal{P}} | \Dec{ \Language{t}}, \VisualObservations{0:t} )$. 
%
The factor is modeled using a vision-language framework \emph{Sentence Tracker} \cite{barbu2013saying}.  
%
The system concurrently performs two inferences. 
%
First, determining the set of grounding symbols from the declarative portion of 
the command. 
%
As an example, the input sentence, ``the block  on the table that the human put down" relates to 
likely grounding predicate symbols  \textsc{Block}(X) $\wedge$ \textsc{Human}(Y) $\wedge$ \textsc{PutDown}(X,Y) $\wedge$ \textsc{Table}(Z) $\wedge$ \textsc{On}(X,Z) where the predicate arguments 
express conditional dependencies from the parse structure. 
%
Similarly, a latent model for tracking is instantiated that 
estimates the spatial and temporally coherent set of detections from percepts. 

%
Declarative groundings including entities and events, such as \textsc{Block}(X) $\wedge$ \textsc{PutDown}(X, Y) $\wedge$ \textsc{Human}(Y), are represented as 
temporal sequence of latent states that explain observations of \emph{trackers}. 
%
The trackers in turn are modeled as sequential models that 
estimate spatio-temporally coherent detection sequences from visual observations $\VisualObservations{0:t}$. 
%
The estimated tracks are associated with semantic entities. 
%
The trackers are constrained by the implied grounding relations from declarative language. 
%
The system is implemented as a Factorial Hidden Markov Model \cite{ghahramani1997factorial} 
used for jointly estimating the groundings and object tracking. 
%
Overall, the model estimates grounding for 
declarative language and accounts for uncertainty in the perception process.

%The determination of tracks ($P( \WorldModel{t} | \Dec{ \Language{t}}, \VisualObservations{0:t})$) and the 
%conditional likelihood of entity or action relations 
%($P( \Correspondences{t}^{\mathcal{P}} | \Dec{ \Language{t}}, \WorldModel{t} )$) is performed jointly as factored HMMs. For a detailed exposition please see \cite{barbu2013saying}. 

Note that performing inference and propagating the full space of declarative groundings is computationally challenging.  
The formulation above allows delayed inference. The declarative component of the command instantiates a focused 
inference process over all past observations $\VisualObservations{0:t}$ to determine the restricted 
set of likelihoods required for the input command. As discussed in Section~\ref{sec:ca} this approach increases inference time for
incremental estimation but eliminates the need to determine the truth of all possible declarative groundings. Moreover,
inference is performed in the context of performing a task thereby increasing the reliability of
poorly performing visual detectors.

%%%% ATTIC %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
% Declarative factor: factorisation over the phrases.
\begin{equation} \label{eq:dec-language-factorisation}
\begin{split}
  \prod_{i = 1}^{ | \Dec{ \Language{t}} | }
  \{
  \prod_{j = 1}^{ | \Grounding{t}^{\mathcal{F}} | }
  \P( \CV{ij}^{\mathcal{F}} | \Dec{ \Phrase{i} }, \GV{ij}^{\mathcal{F}}, \Grounding{c_{i}}^{\mathcal{F}} , \KB{t-1} )
  \}
  \{
  \prod_{k = 1}^{ | \Grounding{t}^{\mathcal{P}} | }
  \P( \CV{ik}^{\mathcal{P}} | \Dec{ \Phrase{i} }, \GV{ik}^{\mathcal{P}}, \Grounding{c_{i}}^{\mathcal{P}}, \WorldModel{t} ) 
  \}
  \P( \WorldModel{t} | \Dec{ \Language{t}}, \VisualObservations{0:t} )
\end{split}
\end{equation}

% Factored over groundings types
\begin{equation} \label{eq:dec-factor-types}
\begin{split}
  \prod_{i = 1}^{ \Dec{n} }
  \left(
  \prod_{j = 1}^{ \Grounding{}^{ \mathcal{S} \cup \mathcal{D} } (\WorldModel{t}) }
    P( \Dec{ \CV{ij} } | \Dec{ \Phrase{ij} }, \Dec{ \GV{ij} }, \Dec{ \Correspondences{ c_{ij} } }, \WorldModel{t} )
  \right)
  \left(
  \prod_{k = 1}^{ \Grounding{}^{ \mathcal{F} } ( \WorldModel{t} ) }
    P( \Dec{ \CV{ik} } | \Dec{ \Phrase{ik} }, \Dec{ \GV{ik} }, \Dec{ \Correspondences{ c_{ik} } },  \KB{t-1} )
  \right)
\end{split}
\end{equation}
\end{comment}

% DCG
\subsubsection{Imperative Grounding Model}
The factor  $P( \Imp{ \Correspondences{t} } | \Imp{ \Language{t} } , \Dec{ \Correspondences{t} }, \WorldModel{t})$ 
estimates the symbolic goals and constraints implied by the imperative instruction given a world model 
and declarative references within the sentence. The constraints inferred from an instruction are provided to a 
a robot planner for execution.
This factor is realized using the \emph{Distributed Correspondence Graph} (DCG) model \cite{howard2014efficient,Paul-RSS-16} 
that efficiently determines the goal objectives (the object(s) to act upon) 
and motion constraints (contact, proximity, visibility etc.) from language instructions.  
For example, utterance like, ``lift the farthest block on the right'' or ``pick up the the can in front of the box" 
result in contact constraint for the robot with an object that displays spatial properties and relations implied in the 
sentence. Additionally, the model allows efficient estimation of aggregate constraints that require hierarchical reasoning over possible objectives e.g. implied in sentences like, ``Pick up the can and the box". 
Formally, the imperative grounding factor can be expressed as:
% Factored over groundings.
\vspace{-1.5ex}
\begin{equation} \label{eq:imp-cv-full}
\begin{split}
P( \Imp{ \Correspondences{t} } |  \Imp{ \Language{t} }, \Dec{ \Correspondences{t} }, \WorldModel{t} ) = 
  \prod_{i = 1}^{ \Imp{\Language{t}} }
  \prod_{j = 1}^{ | \Imp{ \Grounding{} } (\WorldModel{t}) | }
    P( \Imp{ \CV{ij} } | \Imp{ \Phrase{i} }, \Imp{ \GV{ij} }, \Imp{ \Grounding{c_{ij} } }, \Dec{ \Correspondences{t} }, \WorldModel{t} )
\end{split}
\end{equation}

The joint distribution factors hierarchically over $\lambda_{i} \in \Imp{\Language{t}}$ phrases as determined by the parser. Here, $\Imp{\Grounding{c_{ij}}}$ denotes the grounding for child phrases in the instruction. 
Importantly, the conditioning on true declarative correspondences $\Dec{\Correspondences{t}}$ from child phrases 
serves as a link between the imperative and declarative grounding models. 
The probabilistic linkage allows disambiguation of action objectives based on stated declarative knowledge in the 
instruction. Consider the utterance ``pick up the block that the human put down" where a specific block from a number of blocks is implied for manipulation. 

Each grounding factor in the model is expressed as a log-linear model with feature functions that exploit lexical cues, spatial characteristics and the context of child groundings. 
Inference is posed as a search over binary correspondences and is executed as a beam search.
The ordered sequence of inferred groundings serve as an input to the planner that generates a platform-specific motion plan to satisfy the objective.



==> sections/factors-sentence-tracker.tex <==
% Sentence Tracker Factor
\subsubsection{The Sentence Tracker Model}
Add an intro statement here if required.

% Sentence Tracker Figure.
\begin{figure}
  \centering
  \scalebox{0.6}{
  \begin{tikzpicture}
    % detections
    \node[obs] (d1p1) {$\VisualObservations{t-1}$};
    \node[obs, right=of d1p1] (d2p1) {$\VisualObservations{t}$};
    \node[obs, right=of d2p1] (d3p1) {$\VisualObservations{t+1}$};
    \node[left=of d1p1] {\ldots};
    \node[right=of d3p1] {\ldots};
    % trackers
    \node[latent, above=of d1p1] (r1p1) {$\Tracker[t-1][\NumTrackers]$};
    \node[latent, above=of r1p1] (r1p2) {$\Tracker[t-1][0]$};
    \node[latent, right=of r1p1] (r2p1) {$\Tracker[t\phantom{-1}][\NumTrackers]$};
    \node[latent, right=of r1p2] (r2p2) {$\Tracker[t\phantom{-1}][0]$};
    \node[] (rdots) at ($(r2p1)!0.55!(r2p2)$) {\vdots};
    \node[latent, right=of r2p1] (r3p1) {$\Tracker[t+1][\NumTrackers]$};
    \node[latent, right=of r2p2] (r3p2) {$\Tracker[t+1][0]$};
    \edge{r1p1}{r2p1}; \edge{r2p1}{r3p1};
    \edge{r1p2}{r2p2}; \edge{r2p2}{r3p2};
    \edge[bend left=32]{r1p1}{d1p1}; \edge[bend left=32]{r2p1}{d2p1}; \edge[bend left=32]{r3p1}{d3p1};
    \node[left=of r1p1] (or1p1) {\ldots}; \edge{or1p1}{r1p1};
    \node[left=of r1p2] (or1p2) {\ldots}; \edge{or1p2}{r1p2};
    \node[right=of r3p1] (or3p1) {\ldots}; \edge{r3p1}{or3p1};
    \node[right=of r3p2] (or3p2) {\ldots}; \edge{r3p2}{or3p2};
    % words
    \node[latent, above=of r1p2] (w1p1) {$\GroundingFactored[t-1][\NumDecGroundings]$};
    \node[latent, above=of w1p1] (w1p2) {$\GroundingFactored[t-1][0]$};
    \node[latent, right=of w1p1] (w2p1) {$\GroundingFactored[t\phantom{-1}][\NumDecGroundings]$};
    \node[latent, right=of w1p2] (w2p2) {$\GroundingFactored[t\phantom{-1}][0]$};
    \node[] (wdots) at ($(w2p1)!0.55!(w2p2)$) {\vdots};
    \node[latent, right=of w2p1] (w3p1) {$\GroundingFactored[t+1][\NumDecGroundings]$};
    \node[latent, right=of w2p2] (w3p2) {$\GroundingFactored[t+1][0]$};
    \edge{w1p1}{w2p1}; \edge{w2p1}{w3p1};
    \edge{w1p2}{w2p2}; \edge{w2p2}{w3p2};
    \edge[bend left=32]{w1p1}{r1p1,r1p2}; \edge[bend left=32]{w2p1}{r2p1,r2p2}; \edge[bend left=32]{w3p1}{r3p1,r3p2};
    \edge[bend right=32]{w1p2}{r1p1,r1p2}; \edge[bend right=32]{w2p2}{r2p1,r2p2}; \edge[bend right=32]{w3p2}{r3p1,r3p2};
    \node[left=of w1p1] (ow1p1) {\ldots}; \edge{ow1p1}{w1p1};
    \node[left=of w1p2] (ow1p2) {\ldots}; \edge{ow1p2}{w1p2};
    \node[right=of w3p1] (ow3p1) {\ldots}; \edge{w3p1}{ow3p1};
    \node[right=of w3p2] (ow3p2) {\ldots}; \edge{w3p2}{ow3p2};
    \edge[bend left=35]{r1p2}{d1p1}; \edge[bend left=35]{r2p2}{d2p1}; \edge[bend left=35]{r3p2}{d3p1};
  \end{tikzpicture}
}
\caption{Sentence tracker diagram.}
\end{figure}


% More accessible figure
% COMMENTING OUT NOW FOR SPACE
\begin{comment}
\begin{figure}
  \centering
    \scalebox{0.6}{
    \begin{tikzpicture}[scale=7]
      \node[] (Claire) at (0.5,0.7) {\lightBlue person\strut};
      \node[] (and) at ($(Claire.east)+(0.1em,0)$) {\grey \strut};
      \node[] (Bill) at ($(and.east)+(0.1em,0)$) {\lightBlue person\strut};
      \node[] (moved) at ($(Bill.east)+(0.2em,0)$) {\lightBlue moved\strut};
      \node[] (a) at ($(moved.east)+(0.04em,0)$) {\grey \strut};
      \node[] (chair) at ($(a.east)+(0.14em,0)$) {\lightBlue chair\strut};
      \node[] (agent1) at (0.4, 0.45) {{\red $\text{agent}_1$-track}};
      \node[] (agent2) at (0.8, 0.45) {{\red $\text{agent}_2$-track}};
      \node[] (patient) at (1.2, 0.45) {{\red patient-track}};
      \node[] (neqA) at (0.3,0.7) {\lightBlue $\neq$\strut};
      \draw[-] ($(neqA.south)$) -- ($(agent1.north)-(0.08em,0)$);
      \draw[-] ($(neqA.south)$) -- ($(agent2.north)-(0.08em,0)$);
      \draw[-] ($(Claire.south)$) -- ($(agent1.north)+(-0.04em,0)$);
      \draw[-] ($(Bill.south)$) -- ($(agent2.north)+(-0.04em,0)$);
      \draw[-] ($(chair.south)$) -- ($(patient.north)+(0.04em,0)$);
      \draw[-] ($(moved.south)$) -- ($(agent1.north)$);
      \draw[-] ($(moved.south)$) -- ($(patient.north)$);
      \draw[-] ($(moved.south)$) -- ($(agent1.north)$);
      \draw[-] ($(moved.south)-(0,0.03em)$) -- ($(patient.north)-(0.2em,0)$);
      \draw[-] ($(moved.south)-(0,0.03em)$) -- ($(agent2.north)$);
    \end{tikzpicture}}
  \caption{An idea for a ST figure}
\end{figure}
\end{comment}

% Declarative groundings section
\subsubsection{Estimating Declarative Groudings}
Factor. $ \P( \Dec{ \Correspondences{t} }, \Dec{ \Language{t} }, \Dec{ \Correspondences{t} }, \KB{t-1}, \WorldModel{t} ) $

% Declarative factor: factorisation over the phrases.
\begin{equation} \label{eq:dec-language-factorisation}
\begin{split}
P( \Dec{ \Correspondences{t} } |  \Dec{ \Language{t} } , \KB{t-1}, \WorldModel{t} ) = 
  \prod_{i = 1}^{ \Dec{n} }
    P( \Dec{ \CV{i} } | \Dec{ \Phrase{i} }, \Dec{ \GV{i} }, \Dec{ \Grounding{c_{i} } }, \KB{t-1}, \WorldModel{t} )
\end{split}
\end{equation}

% Factored over groundings.
\begin{equation} \label{eq:dec-cv-full}
\begin{split}
P( \Dec{ \Correspondences{t} } |  \Dec{ \Language{t} } , \KB{t-1}, \WorldModel{t} ) = 
  \prod_{i = 1}^{ \Dec{n} }
  \prod_{j = 1}^{ \Dec{ \Grounding{} } (\WorldModel{t}) }
    P( \Dec{ \CV{ij} } | \Dec{ \Phrase{ij} }, \Dec{ \GV{ij} }, \Dec{ \Correspondences{ c_{ij} } },  \KB{t-1} , \WorldModel{t} )
\end{split}
\end{equation}

% Factored over groundings types
\begin{equation} \label{eq:dec-factor-types}
\begin{split}
  \prod_{i = 1}^{ \Dec{n} }
  \left(
  \prod_{j = 1}^{ \Grounding{}^{ \mathcal{S} \cup \mathcal{D} } (\WorldModel{t}) }
    P( \Dec{ \CV{ij} } | \Dec{ \Phrase{ij} }, \Dec{ \GV{ij} }, \Dec{ \Correspondences{ c_{ij} } }, \WorldModel{t} )
  \right)
  \left(
  \prod_{k = 1}^{ \Grounding{}^{ \mathcal{F} } ( \WorldModel{t} ) }
    P( \Dec{ \CV{ik} } | \Dec{ \Phrase{ik} }, \Dec{ \GV{ik} }, \Dec{ \Correspondences{ c_{ik} } },  \KB{t-1} )
  \right)
\end{split}
\end{equation}

Note: The space of declarative grounding symbols relates to objects, events and facts. 
The space of groundings is a function of the world model. The set of objects are used to 
propositionalise predicates (notion of a block) to form the space of groundings 
(all the instances of blocks in the workspace).  

Factored HMM model for declarative groundings.
% Notation for Word HMM
\begin{itemize}
\item Let $\NumDecGroundings$ denote the number of declarative grounding predicates. 
\item Let $\GroundingFactored[t][i]$ represent the state of a grounding tracker. It consists of 
a multinomial ranging over one of $\NumTrackers$, each indicating an inferred track.
Let $\GroundingFullState{t}$ denote the full state of grounding trackers consisting of the set
$\{ \GroundingFactored[t][0], \dots , \GroundingFactored[t][\NumDecGroundings] \}$.
\end{itemize}
 
% Standard Word HMM. 
\begin{equation} \label{eq:hmm-a-full-state}
\begin{split}
P( \GroundingFullState{t} | \TrackerFullState{0:t} ) = 
P(\GroundingFullState{0})
  \bigg[ 
    \prod_{t' = 1}^{t} P( \GroundingFullState{t'} | \GroundingFullState{t'-1} ) P( \TrackerFullState{t'} | \GroundingFullState{t'} ) 
  \bigg]
\end{split}
\end{equation}

% Standard HMM Expanded 
\begin{equation} \label{eq:hmm-a-full-state-expanded}
\begin{split}
%P( \GroundingFullState{t} | \TrackerFullState{0:t} ) = 
P( \GroundingFactored[0][0], \dots, \GroundingFactored[0][\NumDecGroundings] ) = \\
  \Bigg\{
    \prod_{t' = 1}^{t} 
      P(  \GroundingFactored[t'][0], \dots, \GroundingFactored[t'][\NumDecGroundings] \} | \{ \GroundingFactored[t'-1][0], \dots \GroundingFactored[t'-1][\NumDecGroundings] )
      P(  \Tracker[t'][1], \dots, \Tracker[t'][\NumTrackers] | \{ \GroundingFactored[t'][0], \dots, \GroundingFactored[t'][\NumDecGroundings] ) 
  \Bigg\}
\end{split}
\end{equation}

% Factored HMM
\begin{equation} \label{eq:hmm-a-factored}
\begin{split}
%P( \GroundingFullState{t} | \TrackerFullState{t0:} ) = 
P( \GroundingFactored[0][0], \dots, \GroundingFactored[0][\NumDecGroundings] ) = 
\bigg\{ 
\prod_{m=1}^{\NumDecGroundings}
P( \GroundingFactored[0][m] ) 
\bigg\}
    \Bigg\{ 
      \prod_{t' = 1}^{t} 
      \bigg\{ 
        \prod_{m = 1}^{\NumDecGroundings} P( \GroundingFactored[t'][m] | \GroundingFactored[t'-1][m] ) 
      \bigg\}
      P( \TrackerFullState{t'} | \GroundingFullState{t'} ) 
    \Bigg\}
\end{split}
\end{equation}

% Factored HMM
\begin{equation} \label{eq:hmm-a-factored-expanded}
\begin{split}
%P( \GroundingFullState{t} | \TrackerFullState{0:t} ) = 
%P( \GroundingFactored[0][0], \dots, \GroundingFactored[0][\NumDecGroundings] ) = 
\bigg\{ 
  \prod_{m=1}^{\NumDecGroundings} P( \GroundingFactored[0][m] )
\bigg\} 
    \Bigg\{ 
      \prod_{t' = 1}^{t} 
      \bigg\{ 
        \prod_{m = 1}^{\NumDecGroundings} P( \GroundingFactored[t'][m] | \GroundingFactored[t'-1][m] ) 
      \bigg\} %\\
      P( \Tracker[t'][1], \dots, \Tracker[1][\NumTrackers] | \GroundingFactored[t'][1], \dots, \GroundingFactored[t'][\NumDecGroundings] ) 
    \Bigg\}
\end{split}
\end{equation}

% Factored HMM
\begin{equation} \label{eq:hmm-a-factored-expanded}
\begin{split}
%P( \GroundingFullState{t} | \TrackerFullState{0:t} ) = 
%P( \GroundingFactored[0][0], \dots, \GroundingFactored[0][\NumDecGroundings] ) = \\
\bigg\{ 
  \prod_{m=1}^{\NumDecGroundings} P( \GroundingFactored[0][m] )
\bigg\} 
    \Bigg\{ 
      \prod_{t' = 1}^{t} 
      \bigg\{ 
        \prod_{m = 1}^{\NumDecGroundings} P( \GroundingFactored[t'][m] | \GroundingFactored[t'-1][m] ) 
      \bigg\} 
      \prod_{k=1}^{\NumTrackers}
      P( \Tracker[t'][k]| pred(\GroundingFactored[t'][1], \dots, \GroundingFactored[t'][\NumDecGroundings]) ) 
    \Bigg\}
\end{split}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%% World Model Estimation
\subsubsection{Estimating World Model}
The factor, $\P( \WorldModel{t}, \VisualObservations{0:t} )$

% Notation for HMM
\begin{itemize}
\item Image at time $t$ denoted as $\Image{t}$
The set of detections derived from $\Image{t}$ at time $t$ is denoted as 
$ \VisualObservations{t} = \{ \VisualObservation[t][0], \dots, \VisualObservation[t][n_t] \} $ 
The set of observations $\VisualObservations{0:t} = \{ \VisualObservations{0}, \dots,  \VisualObservations{t} \}$ 
derived from $\Images{0:t}$.
\item Let $\NumTrackers$ be the number of trackers derived from the declarative langauge $\Dec{ \Language{t}}$.
\item Let $\Tracker[t][i]$ represent a tracker state consisting of a multinomial ranging over one of  
$\NumDetections$ indices, each indicating an image detection.
Let $\TrackerFullState{t}$ denote the full state of trackers consisting of the set
$\{ \Tracker[t][0], \dots , \Tracker[t][\NumTrackers] \}$.
\end{itemize}
 
% Standard HMM. 
\begin{equation} \label{eq:hmm-a-full-state}
\begin{split}
P( \TrackerFullState{t} | \VisualObservations{0:t} ) = 
P(\TrackerFullState{0})
  \bigg[ 
    \prod_{t' = 1}^{t} P( \TrackerFullState{t'} | \TrackerFullState{t'-1} ) P( \VisualObservations{t'} | \TrackerFullState{t'} ) 
  \bigg]
\end{split}
\end{equation}

% Standard HMM Expanded 
\begin{equation} \label{eq:hmm-a-full-state-expanded}
\begin{split}
P( \TrackerFullState{t} | \VisualObservations{0:t} ) = 
P( \Tracker[0][0], \dots, \Tracker[0][\NumTrackers] ) \\
  \Bigg\{
    \prod_{t' = 1}^{t} 
      P(  \Tracker[t'][0], \dots \Tracker[t'][\NumTrackers] \} | \{ \Tracker[t'-1][0], \dots \Tracker[t'-1][\NumTrackers] ) 
      P(  \VisualObservation[t'][1], \dots, \VisualObservation[t'][\NumDetections] | \{ \Tracker[t'][0], \dots \Tracker[t'][\NumTrackers] ) 
  \Bigg\}
\end{split}
\end{equation}

% Factored HMM
\begin{equation} \label{eq:hmm-a-factored}
\begin{split}
P( \TrackerFullState{t} | \VisualObservations{0:t} ) = 
\bigg\{ 
\prod_{m=1}^{\NumTrackers}
P( \Tracker[0][m] ) 
\bigg\}
    \Bigg\{ 
      \prod_{t' = 1}^{t} 
      \bigg\{ 
        \prod_{m = 1}^{\NumTrackers} P( \Tracker[t'][m] | \Tracker[t'-1][m] ) 
      \bigg\}
      P( \VisualObservations{t'} | \TrackerFullState{t'} ) 
    \Bigg\}
\end{split}
\end{equation}

% Factored HMM
\begin{equation} \label{eq:hmm-a-factored-expanded}
\begin{split}
P( \TrackerFullState{t} | \VisualObservations{0:t} ) = 
\bigg\{ 
  \prod_{m=1}^{\NumTrackers} P( \Tracker[0][m] )
\bigg\} \\
    \Bigg\{ 
      \prod_{t' = 1}^{t} 
      \bigg\{ 
        \prod_{m = 1}^{\NumTrackers} P( \Tracker[t'][m] | \Tracker[t'-1][m] ) 
      \bigg\}
      P( \VisualObservation[t'][1], \dots, \VisualObservation[t'][\NumDetections] | 
         \Tracker[t'][1], \dots, \Tracker[1][\NumTrackers] ) 
    \Bigg\}
\end{split}
\end{equation}



==> sections/problem-statement.tex <==
\section{Problem Formulation} 
\label{sec:problem-Fomulation}
%% Informally, introduce the problem to solve.
Our goal is to allow the robot to ground instructions that involve 
reasoning over knowledge acquired from past observations and 
factual knowledge communicated by the human.
%
As an example, consider the scenario where the robot observes a human put down a box and the 
can in its workspace populated with a number of objects. 
%
The human states that, ``the can and the box that I put down are my snack" and then instructs the robot to 
``pack up my snack" desiring the robot to manipulate the two indicated objects.  

%% Notation
% Language
The robot receives language inputs $\Language{0:t}$ from the human operator that convey 
either a command or convey facts that may be relevant for interpreting a later command.  
Let $\Images{0:t}$ denote the set of images received till time $t$.
We assume the presence of an object detection and classification system for an \emph{apriori} 
known set of object classes which yields potential detections, each a sub-image, with an associated 
class likelihood. Let $\VisualObservations{t}$ denote the set of detections 
$ \{ \VisualObservation[t][0], \dots,\VisualObservation[t][n_{t}] \}$ from $\Image{t}$ 
where $n_{t}$ is the total number of detections obtained in the image.
The cumulative set of detections from images $\Image{0:t}$ forms the observation set
$\VisualObservations{0:t} = \{ \VisualObservations{0}, \dots, \VisualObservations{t} \}$.
Interpreting instructions with past visual and linguistic observations can be posed as: 
% Over time.
\begin{equation} \label{eq:joint-dist-all-context}
 P( \Control, \Correspondences{t} | \Language{0:t}, \VisualObservations{0:t} )  
\end{equation}

% World Model
Here, we relax the assumption of a known world representation ahead of time, 
and instead aim to acquire the relevant representation from past percepts.
%
We assume a notion of objects as a set of visually and temporally coherent set of detections. 
% Grounding.
Hence, we incorporate a generalised notion of groundings $\Grounding{t}$ 
as probabilistic predicates. 
% 
This encodes the uncertainty in process of inferring 
entities (such as objects and agents in the scene)and the associated uncertainty in 
relationships between them.
% Correspondences
Further, correspondence variables relate language to a space of concepts as informed by the robot's 
observations. 

% Why it is hard.
Learning the distribution in Equation \ref{eq:joint-dist-all-context} challenging due to two reasons.
Firstly, grounding the current command given the full set of past visual-linguistic
observations involves learning a conditional distribution defined over the
space of potential groundings for past commands that grows combinatorially with increasing context.
We address the issue of maintaining an appropriate representation
of past observations in the Section \ref{sec:pgm}.
Secondly, estimating directly with percepts rather than a known semantic world model
leads to an exponential increase in the space of potential groundings since
a multitude hypotheses for potential entities may exist.
In Section \ref{sec:factors}, we demonstrate how a relevant world model for the command is estimated.



==> sections/related-works.tex <==
\section{Related Work}
\label{sec:related-work}

\todo[inline]{Revise.}
% Traditional symbol grounding.

Symbol grounding in robotics can be largely divided into two streams of work,
those that assume a fixed known world model and those that infer the world model
while grounding symbols.
%
Approaches such as those of
\citet{tellex2011understanding,howard2014efficient,chung2015performance,Paul-RSS-16}
relate input language to entities in the world and actions to be performed by
the robot by structuring their inference according to the parse or semantic
structure embedded in language.
%
They take advantage of a known world model to further constrain inference and
consider a command to be interpreted in a static world.
%
Moreover they use no intermediate representation and directly produce the
groundings and action to be performed but are unable to remember facts and
incorporate knowledge about prior actions performed by other agents.
%
A related set of approaches, such as those of
\citet{zettlemoyer2007online,chen2010training,kim2012unsupervised,berant2013freebase,artzi2013weakly}
employ semantic parsing to convert a command to an intermediate representation,
either $\lambda$-calculus or a closely related formalism, which can then be
executed by a robot.
%
\citet{kirk2016learning} learn to determine the goals of commands by visual
observation, a closely related task to command following, and then ground those
commands in perception.
%
This prior work assumes that the world state is deterministic, although
partially-observable, that facts are known with precision, and that they are not
retracted or invalidated.
% 
The above models assume the presence of a world model populated with semantic
entities that usually comes from a semantic mapping process
\cite{pronobis2012large}.
% 
These models preform unidirectional inference where the grounding process
reasons about intended tasks and constraints based on a single point estimate of
its understanding of the world.

% Those who relax the assumptions. 
\citet{MatuszekAAAI2014} present a formulation that allows uncertainty in
knowledge about object models in the scene and present a model that allows
learning object attributes and spatial relations through joint reasoning with
perceptual features and language information.
%
\citet{chen2011learning} take a similar approach to learn actions from map
features for input language.
%
The work of \citet{hemachandra15,walter14a} incorporates language as an
additional sensor while building a map of the environment using camera and LIDAR
data and infers a semantic representation by reasoning in the joint space.
%
\citet{guadarrama2013grounding} demonstrate a system that integrates visual and
spatial information with semantic parsing to interpret actions and ground
spatial relations.
% Limitation.
However, in all of these approaches inference is restricted to attributes that
are unary predicates or at most static binary spatial relations between
objects.
%
These model do not reason about either higher-order actions or changing spatial
relations such as activities or relations between collections of objects such as
groups.
% Persistence
A common limitation of existing symbol grounding approaches is that inferred
groundings are based on the current state or consider only a short-horizon
history of the world model.
%
Further, the history contains a simplistic representation like objects,
constraints and regions and does not include non-perceptual facts or
higher-order knowledge about events or entities in the world.
%
Maintaining and updating a rich representation of the world model over time and
simultaneously inferring intended actions remains a technical gap that we
address in this work.

% There's no room for a review of NLP or Vision!
% Vision and Knowledge representations.
%%% Commenting out for space.
\begin{comment}
Vision approaches attempt to infer higher-order information from image or 
video streams (examples). Systems like the Sentence tracker \cite{barbu2013saying} jointly reason with language and percepts to infer higher-order behaviors. 
Cite others: visual question answering \cite{agrawal2015vqa}, word2vec \cite{kottur2015visual} etc.
Traditional knowledge representation systems like START system 
\cite{katz1988using}
%\cite{katz1988using,katz1997annotating,katz2002omnibase} 
store and organise relational knowledge about the world. Cite other data bases or ontologies like Cyc etc.
The above systems 
learn and store higher order information present in the world model but do not incorporate inferring 
intent and plans that the agent can take in the future. 
\end{comment}


==> sections/technical-approach.tex <==
\section{Technical Approach}
\label{sec:technical-approach}

\subsection{Symbolic Representation}
We formally define the symbolic representation.
Expand the scope of symbls. 
Emphasise, actions and arbitrary facts. Classes of symbols.

\subsection{Integrating Past Visual-Linguistic Context}

\begin{equation}
\begin{split}
 P( \Correspondences{t+1},  | \Language{0:t+1}, \VisualObservations{0:t} ) = \\ 
 \Integral{ \KB{t} }
 P( \Correspondences{t+1} | \Language{t+1}, \VisualObservations{0:t}, \KB{t} )  
 P( \KB{t} | \Language{0:t}, \VisualObservations{0:t} ) 
\end{split}
\end{equation}


\subsection{Estimation Framework}

\begin{equation} \label{eq:target-joint}
 P( X_{t+1}(t') | \Lambda_{0:t+1}, Z_{0:t} )
\end{equation}

\begin{equation} \label{eq:target-joint-phi}
 \Integral{\Phi_{t+1} }
 P( X_{t+1}(t') | \Phi_{t+1} ) P( \Phi_{t+1} | \Lambda_{0:t+1}, Z_{0:t} )
\end{equation}

\begin{equation} \label{eq:target-joint-kb}
\begin{split}
 P( \Phi_{t+1} | \Lambda_{0:t+1}, Z_{0:t} ) = P( \Phi_{t+1} | \Lambda_{t+1}, \Lambda_{0:t}, Z_{0:t} ) \\
 = 
 \Integral{ \nu_{t} } 
 P( \Phi_{t+1} | \Lambda_{t+1}, Z_{0:t}, \nu_{t} ) 
 P( \nu_{t} | \Lambda_{0:t}, Z_{0:t} )
\end{split}
\end{equation}

%\begin{equation} \label{eq:target-kb-recursive}
%\begin{split}
%bel( \nu_{t} ) =  P( \nu_{t} | \Lambda_{0:t}, Z_{0:t} )  \\
%= \Integral{ \nu_{t-1} } P( \nu_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} ) P( \nu_{t-1} | \Lambda_{0:t-1}, Z_{0:t-1} ) \\
%= \Integral{ \nu_{t-1} } P( \nu_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} ) bel( \nu_{t-1} )
%\end{split}
%\end{equation}

\begin{equation} \label{eq:target-kb-recursive}
\begin{split}
 P( \nu_{t} | \Lambda_{0:t}, Z_{0:t} )  
 = \Integral{ \nu_{t-1} } P( \nu_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} ) \\ P( \nu_{t-1} | \Lambda_{0:t-1}, Z_{0:t-1} ) \\
\end{split}
\end{equation}

Let $bel( \nu_{t} )$ denote $P( \nu_{t} | \Lambda_{0:t}, Z_{0:t} )$ and can be computed recursively as:

\begin{equation} \label{eq:target-kb-recursive}
\begin{split}
  bel( \nu_{t} ) = \Integral{ \nu_{t-1} } P( \nu_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} ) bel( \nu_{t-1} )
\end{split}
\end{equation}

The incremental estimation problem stated above requires the computation of the 
following two quantities:
\begin{enumerate}[label=(\roman*)]
  \item $P( \Phi_{t+1} | \Lambda_{t+1}, Z_{0:t}, \nu_{t} )$: estimating the grounding 
        for a command given the current knowledge base and visual observations, and 
  \item $P( \nu_{t} | \Lambda_{t}, Z_{0:t}, \nu_{t-1} )$: the belief update for the 
        knowledge base given the language input and observations. 
\end{enumerate}
We pose the estimation of these two quantities as inference on a graphical model 
which is presented next. 



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


